Flowette: Flow Matching with Graphette Priors for Graph Generation

We study generative modeling of graphs with recurring subgraph motifs. We propose Flowette, a continuous flow matching framework that employs a graph neural network-based transformer to learn a velocity field over graph representations with node and edge attributes. Our model promotes topology-aware alignment through optimal transport-based coupling and preserves structural fidelity through endpoint- and chemistry-aware regularisation. To incorporate domain-driven structural priors, we introduce graphettes, a new probabilistic family of graph structure models that generalize graphons via controlled structural edits for motifs such as rings, stars, and trees. We theoretically analyze the coupling, invariance, and structural properties of the framework, evaluate it on synthetic and molecular benchmarks, and isolate the contributions of the structural prior, the optimal-transport coupling, and the regularisation terms through controlled ablations. Flowette achieves competitive performance overall, attaining state-of-the-art results on several metrics across multiple benchmarks, highlighting the effectiveness of combining structural priors with flow-based training for modeling complex graph distributions.

==> NeurIPS_Submission/appeal.tex <==
Reference 1
-----
Reference number or identifier in your paper: 57

Exact citation as it appears in the outcome of the citation checker:
H. Shirzad, H. Hajimirsadeghi, A. H. Abdi, and G. Mori. Td-gen: Graph generation with tree decomposition. Proceedings of the 25th International Conference on Artificial Intelligence and Statistics (AISTATS 2022).

Link to a public authoritative source for the citation format you used. Examples may include the publisher's website, official conference proceedings, journal page, arXiv, google scholars:
https://proceedings.mlr.press/v151/shirzad22a/shirzad22a.pdf

Basis for your appeal:
We acknowledge that the publication venue in this citation is incorrect. However, the referenced work itself is genuine: the title, authors, and year identify the existing TD-GEN paper. The authoritative PMLR record confirms that Hamed Shirzad, Hossein Hajimirsadeghi, Amir H. Abdi, and Greg Mori published TD-GEN: Graph Generation Using Tree Decomposition at AISTATS 2022. Therefore, the error concerns the publication venue rather than the existence or authorship of the cited work. Under the provided criteria, an incorrect venue that nevertheless exists is a minor bibliographic error and should not cause the reference to be classified as hallucinated.

Reference 2
-----
Reference number or identifier in your paper: 56

Exact citation as it appears in the outcome of the citation checker:
Omar Mahmood, Elman Mansimov, Richard Bonneau, and Kyunghyun Cho. Masked graph modeling for molecule generation. Nature communications, 2021.

Link to a public authoritative source for the citation format you used. Examples may include the publisher's website, official conference proceedings, journal page, arXiv, google scholars:
https://www.nature.com/articles/s41467-021-23415-2

Basis for your appeal:
We acknowledge that this reference contains incorrect bibliographic metadata. However, we respectfully request reconsideration of its classification as a hallucinated reference. The cited title, "Masked Graph Modeling for Molecule Generation", corresponds to a genuine and publicly verifiable publication. This reference was added at a late stage of manuscript preparation to strengthen the introduction and related work. Unfortunately, during this process, its bibliographic information was inadvertently cross-assigned with that of another genuine work in the same molecular graph generation literature, and we did not identify this error during our final reference checks. We fully acknowledge that this was an honest mistake on our part and that the reference should have been checked more carefully before submission. Importantly, however, the cited publication itself is genuine, identifiable from its title, and directly relevant to the discussion for which it was cited. The error therefore arose from an inadvertent association of metadata between existing publications rather than the fabrication of a nonexistent publication or scientific evidence. We respectfully ask that the nature and circumstances of this error be considered when determining whether this reference should be classified as hallucinated.

==> NeurIPS_Submission/checklist.tex <==
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1--2 sentence) justification right after your answer (even for \answerNA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will also be asked to include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While \answerYes{} is generally preferable to \answerNo{}, it is perfectly acceptable to answer \answerNo{} provided a proper justification is given (e.g., error bars are not reported because it would be too computationally expensive'' or ``we were unable to find the license for the dataset we used''). In general, answering \answerNo{} or \answerNA{} is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The abstract and introduction accurately convey the paper's scope and contributions, clearly outlining the key claims, underlying assumptions, and limitations.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The limitations are discussed under "Observed Limitations" on page 10.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: A complete set of assumptions, theorems, and proofs is provided in Sections 3 and 4, as well as Appendices E and H.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper provides all the information needed to reproduce the main experimental results on pages 8-9, and in Appendix J.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper provides open access to the data and code on page 8. The code is available at: \url{https://github.com/wokas36/Flowette}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, all the training and test details are provided on pages 8-10, and Appendix J.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Mean and standard-deviation is provided in many experimental results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper provides sufficient information on computational resources and runtime characteristics to support reproducibility.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, this work adheres to the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Not required for our work.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not present any such risks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All datasets and models are properly cited and are publicly available.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No new assets introduced.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Not used in our work.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Not required for our work.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Doesn't involve LLMs.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> NeurIPS_Submission/rebuttal_neurips.tex <==
Reviewer3 (8BQw)
----
We sincerely thank for your valuable comments helping improve our work.

***Q1. Node-level alignment induced by FGW is under-specified.***

In Flowette, FGW is used at two distinct levels: the scalar FGW distance $D_{ij}$ is used by the Hungarian algorithm to select graph-level source–target pairs, while the corresponding optimal transport plan $T_{ij}^{*}$ is subsequently used as a soft node-level alignment; it is neither discarded nor converted into a hard permutation. For a selected pair, we row-normalise the coupling to obtain $R_{ab}=\frac{T_{ab}^{\*}}{\sum_{b'}T_{ab'}^{\*}},$ where $R_{ab}$ represents the correspondence between source node $a$ and target node $b$. We row-normalise $T^{\*}$ because it represents joint transport mass; normalisation converts each row into a probability distribution over target nodes, preserving feature scale and recovering the exact permutation when the coupling is hard. Before forming any interpolants or velocity targets, the target graph is transported into the source-node coordinate system as, 

$\widetilde{X}_1 = R X_1$, 

$\widetilde{A}_1 = R A_1 R^{T}$, 

$\widetilde{E}_{1,ab:} = \sum\_{ab} R\_{aj} E\_{1,jk:} R\_{bk}$.

The flow is therefore constructed as $G_t=(1-t)G_0+t\widetilde{G}_1$, and the supervised velocities are $\widetilde{A}_1-A_0$, $\widetilde{X}_1-X_0$, and $\widetilde{E}_1-E_0;$ raw target ordering is never directly subtracted from the source ordering. We will revise the Algorithm 6 to explicitly insert this step between tensor construction and interpolation.

***Q2. Endpoint consistency loss may be less independent than claimed.***

We thank the reviewer for this precise observation and agree that our description of $L\_{end}$ as an independent global-consistency signal overstated its independence. Indeed, since $A_t = (1-t) A_0 + t A_1$, $\Delta A = A_1 - A_0$, and $\hat{A}_1 = A_t + (1-t)v_A$, we have $\hat{A}_1-A_1 = (1-t)(v_A-\Delta A)$ with identical relations for node and edge features. Thus, the endpoint term should be interpreted more precisely as an endpoint-aware temporal reweighting of velocity supervision, rather than as an independent source of global information. We will revise Sec. 3.3 to remove the "global transport consistency" framing and instead describe $L\_{end}$ as an algebraically induced, non-uniform temporal reweighting of the same velocity residual.

This reweighting is not arbitrary: the factor $(1−t)^2$ follows directly from the remaining extrapolation horizon in the one-step endpoint estimate, since the same velocity residual induces a larger predicted endpoint error when evaluated earlier in the trajectory. Theorem E.5 separately establishes that endpoint error under $K$-step Euler integration is controlled by velocity approximation error and numerical step size; it does not establish the independence of $L\_{end}$. Therefore, although $L\_{end}$ does not introduce a new supervision target, combining it with $\beta_\{end}$ provides an endpoint-aware temporal reweighting that places greater emphasis on velocity residuals having a larger immediate effect on the predicted terminal state.

***Q3. Runtime and precomputation claims need clarification.***

We support three explicit coupling protocols, and the default protocol Algorithm 1 is online coupling. Thus, the default method does not assume a fixed precomputed source pool. We additionally use two optional amortised variants: fixed-pool, which makes one blockwise pass over the training set before the first epoch, samples one source graph per target, stores the corresponding source graph and FGW transport plan keyed by the target index, and reuses them across all epochs; and periodic, which refreshes this cache every $K$ epochs. Importantly, pre-computation is performed in minibatch-sized $B \times B$ blocks rather than as a single dataset-wide matching problem, and the cached correspondence remains valid under shuffled training because it is indexed by the target graph's dataset index. We will therefore revise the paper to state explicitly those protocols and avoid conflating the default online procedure with the optional amortised version: under online coupling, FGW cost is paid every minibatch and epoch, whereas under fixed-pool coupling it is a one-time preprocessing cost that is reused throughout training.

***Q4. Manual graphette specification and finite-graph approximation.***

The graphette prior could be made more data-driven: the base graphon $W$ could be estimated using graphon learning or implicit neural representation methods, $\rho_n$ could be fitted to match the empirical edge-density scaling conditional on $n$, and the edit distribution $f$ could be learned from motif statistics rather than selected manually. We deliberately use simple, interpretable priors in the present work because the graphette is only the source distribution of the flow, not the final generative model; it is intended to provide a coarse structural bias, such as rings, hubs, or acyclicity, while the velocity field learns the remaining target-specific structure. This also lets us isolate the benefit of structural source bias without introducing a second learned generator.

Sensitivity is partly quantified by our controlled ablation in Appendix J.8.3, where the graphette is replaced by a standard graphon. On QM9, validity and uniqueness decrease from 99.81\% and 99.30\% to 75.50\% and 68.90\%, respectively, while NSPDK increases from 0.0003 to 0.0760; analogous degradation occurs on ZINC250K. This confirms that a structurally compatible prior is important, but we agree that this is an extreme removal ablation rather than a complete misspecification study. 

To further quantify **sensitivity to graphette misspecification**, we performed a controlled experiment as in the following table which all components of Flowette were kept fixed, while only the edit function $f$ was changed. For molecular datasets, the original Flowette prior uses ring addition $R$, reflecting the prevalence of cyclic structures in molecules; we compare it against the structurally incompatible star-addition edit $S$ and the contradictory cycle-deletion edit $h$. The results show a clear and consistent degradation as the prior becomes less compatible with the target domain: on QM9, replacing $R$ with $S$ reduces validity from 99.81\% to 70.50\%, while cycle deletion further reduces it to 53.70\%; analogous trends are observed on ZINC250K, together with substantial increases in NSPDK. This demonstrates that Flowette benefits from a coarse but structurally appropriate source prior and is sensitive to motif misspecification, rather than being invariant to the choice of graphette edit. 
|Dataset|Edit function|Prior variant|Valid|Unique|NSPDK|
|-|-|-|-|-|-|
|QM9|R (Ring addition)|Intended prior|**99.81 $\pm$ 0.09**|**99.30 $\pm$ 0.05**|**0.0003 $\pm$ 0.002**|
||S (Star addition)|Incorrect motif|70.50 $\pm$ 0.06|69.30 $\pm$ 0.06|0.0160 $\pm$ 0.008|
||h (Cycle deletion)|Contradictory motif|53.70 $\pm$ 0.04|54.45 $\pm$ 0.06|0.0540 $\pm$ 0.004|
|ZINC250K|R (Ring addition)|Intended prior|**99.90 $\pm$ 0.10**|**100.00 $\pm$ 0.0**|**0.0006 $\pm$ 0.004**|
||S (Star addition)|Incorrect motif|73.40 $\pm$ 0.06|75.30 $\pm$ 0.06|0.1105 $\pm$ 0.006|
||h (Cycle deletion)|Contradictory motif|51.58 $\pm$ 0.04|50.65 $\pm$ 0.05|0.2050 $\pm$ 0.007|

***Q5. Minor: FGW vs GW.***

We agree that standard GW is sufficient for genuinely non-attributed graphs, and FGW naturally recovers this setting: in Eq. (4), $\alpha=1$ gives GW exactly, while absent or constant node features make the feature term non-discriminative. Our motivation for FGW is therefore not to outperform GW on purely structural datasets, but to provide a unified coupling that also handles attributed graphs. This becomes important for molecules, where topology alone may align structurally similar but chemically incompatible atoms, leading to noisy feature interpolation and velocity targets; FGW resolves this ambiguity by jointly matching topology and atom identity.

To isolate the feature contribution, we compared FGW ($\alpha=0.5$) with GW ($\alpha=1.0$) while keeping all other components fixed. As expected, their performance is essentially identical on the non-attributed Tree and SBM benchmarks: both achieve 100\% validity, uniqueness, novelty, and V.U.N, with only negligible differences in structural MMD metrics. These results confirm that FGW behaves like GW when attributes are uninformative, while retaining the flexibility needed for attributed molecular graphs.

|Dataset|Model Variant|Deg|Clus.|Orbit|Valid|Unique|Novel|V.U.N|
|-|-|-|-|-|-|-|-|-|
|Tree|Flowette (FGW)|0.00005$\pm$ 0.002|0.0000$\pm$ 0.0|0.0000$\pm$ 0.0|100.0$\pm$ 0.0|100.0$\pm$ 0.0|100.0$\pm$ 0.0|100.0$\pm$ 0.0|
||Flowette (GW)|0.00010$\pm$ 0.003|0.0000$\pm$ 0.0|0.0000$\pm$ 0.0|100.0$\pm$ 0.0|100.0$\pm$ 0.0|100.0$\pm$ 0.0|100.0$\pm$ 0.0|
|SBM|Flowette (FGW)|0.0076$\pm$ 0.003|0.0508$\pm$ 0.01|0.0000$\pm$ 0.0|100.0$\pm$ 0.0|100.0$\pm$ 0.0|100.0$\pm$ 0.0|100.0$\pm$ 0.0|
||Flowette (GW)|0.0080$\pm$ 0.005|0.0595$\pm$ 0.03|0.0000$\pm$ 0.0|100.0$\pm$ 0.0|100.0 $\pm$ 0.0|100.0$\pm$ 0.0|100.0$\pm$ 0.0|




Reviewer1 (9NKx)
----
We sincerely thank the reviewer for valuable comments.

***Q1. Why does the velocity-only model perform poorly on molecules?***

Let us clarify an important distinction that Table 8 alone does not fully convey. The poor performance of the ablated variant does not reflect insufficient backbone capacity, it isolates a specific and well-understood mismatch between continuous velocity regression and the discrete, highly constrained nature of molecular graphs. Concretely, a numerically small error in a single bond-type logit can flip a single bond to a double bond, which is enough to violate valence and invalidate an entire molecule, while an error of similar magnitude elsewhere in the same graph is chemically inconsequential. A more expressive GNN can certainly represent the correct velocity field, the issue is not what the model can express, but the regression treats all residuals as equally costly, when chemically they are not.

Crucially, this mismatch is specific to the molecular setting, not a general weakness of our framework. The same backbone - FGW-coupled supervision, the permutation-equivariant GNN transformer, and the rectified flow-matching objective, achieves SOTA results on our synthetic benchmarks (Tree, SBM, Ego-small) with $\beta_{val}=\beta_{atom}=0$ and no chemistry terms whatsoever. The backbone is therefore already domain-general and demonstrably strong on its own; it is only when the target domain has hard combinatorial constraints, like valence, that additional supervision is needed to align the training signal with what correct means in that domain.

Methods like DiGress, DeFoG, and VFM/CatFlow address this problem by building their entire generative process around categorical/discrete state spaces from the ground up. We instead retain the general continuous-flow backbone and attach two lightweight, differentiable regularizers at the predicted endpoint, $L_{val}$ and $L_{atom}$, that penalize exactly the failure mode described above. These require only coarse, easily specified domain knowledge, valence limits and target atom-type marginals, and negligible architectural or computational overhead (Appendix D, F). This is an addition to a general model, not a redesign of it: the coupling mechanism, network architecture, and core flow-matching objective are shared unchanged between our synthetic and molecular experiments, and the domain-specific surface area is confined to these two interpretable terms.

We will revise Sec. 5.2 to state this explicitly: the ablated variant shows that chemical feasibility does not emerge for free from architecture or generic flow-matching supervision alone, evidence that our two chemistry-aware terms are targeted, low-overhead corrections for a specific failure mode, not that the framework is bespoke to molecular data.

***Q2. Misalignment between framing and actual contributions.***

We thank the reviewer for this constructive suggestion and agree that the paper should be framed around its integrated contribution to structurally reliable continuous flow matching for graphs, rather than implying that either graphettes or the backbone alone explains the final performance. Importantly, Flowette retains the same core formulation across synthetic and molecular experiments: FGW-based graph- and node-level coupling, the permutation-equivariant continuous velocity-field GNN, and the flow-matching objectives $L_{vel}$ and $L_{end}$. Domain adaptation occurs only through the coarse graphette edit function and, for molecular datasets, the chemistry-aware regularisers $L_{val}$ and $L_{atom}$.

We will revise the title, introduction, and contribution summary to emphasise three complementary components: (i) graphettes as interpretable structural source priors requiring only coarse domain knowledge, (ii) FGW-based graph- and node-level alignment that provides topology-aware supervision, and (iii) endpoint-aware training with optional domain-specific feasibility regularisation for discrete graph generation. We will explicitly distinguish the reusable, domain-general core-coupling, continuous transport, and the velocity-field architecture from the domain-adaptive prior and chemistry-aware feasibility constraints.

We will also restructure the paper to follow the generative pipeline: graphette construction first, followed by FGW coupling, the continuous flow model, and finally the optional regularisers. This ordering will make clear from the outset which components are shared across domains and which are adapted to a particular task, rather than leaving this distinction to be inferred from the ablations and limitations.

***Q3. What distinguishes GNN backbone from existing graph transformer architectures.***

We thank the reviewer for requesting this clarification. We do claim that the GNN Transformer is a novel architecture. While existing graph transformers operate on fixed discrete states predicting node/edge categories, ours fundamentally differs in three ways: (1) it operates on continuous evolving triple-representations $(A_t, X_t, E_t)$ , predicting velocity fields $(v_A, v_X, v_E)$ rather than categorical outputs; (2) it maintains pairwise edge hidden states with soft adjacency $A_t$ injected as a structural bias in attention logits, absent in existing transformers; and (3) velocity outputs are explicitly symmetrised with time embedding jointly conditioning both node and edge dynamics, unique to continuous flow matching. Together, these make our architecture an original contribution tailored to continuous-time flow matching on attributed graphs.

**(1) Joint continuous graph state and direct velocity prediction.**  Flowette operates on the continuously relaxed graph state $G_t=(A_t,X_t,E_t)$ and directly predicts the coupled velocity field $v_\theta(G_t,t)=(v_A,v_X,v_E)$, where adjacency, node attributes, and edge attributes evolve simultaneously. These outputs are tangent directions that are repeatedly evaluated and integrated by the ODE solver, rather than categorical clean-state logits, endpoint probabilities, or discrete transition rates. The network must therefore remain meaningful throughout the continuum of fractional graph states encountered during generation, not only at discrete valid graphs.

**(2) Explicit separation of evolving topology and edge attributes.**  
Flowette treats soft connectivity $A_t(i,j)$ and edge attributes $E_t(i,j)$ as related but distinct evolving variables. The current soft adjacency is inserted directly into the attention logits, $S_{ij}^{(\ell)} = \frac{\langle Q_i^{(\ell)},K_j^{(\ell)}\rangle}{\sqrt{H}} + A_t(i,j)$, so the evolving topology continuously modulates information exchange. In parallel, a separate pairwise hidden state $b_{ij}^{(\ell)}$, initialised from $E_t$, participates in message construction and is updated at every layer. Thus, $A_t$ controls where and how strongly nodes communicate, while the pairwise state represents what edge-specific information is exchanged. This separation is particularly relevant for molecular graphs because bond existence and bond type are strongly related but are not identical variables.

**(3) Time conditions the complete topology–attribute dynamics.**  
The time embedding is injected into both node and pairwise representations, allowing the interaction between topology and attributes to change throughout transport. Near $t=0$, the field performs coarse transformations from a graphette-prior sample, whereas near $t=1$, it performs finer structural and attribute corrections. Time therefore does not merely serve as a denoising-step index; it conditions a single continuous vector field whose outputs define the right-hand side of the graph ODE.

**(4) Coupled and graph-consistent infinitesimal updates.**  
The final node states predict $v_X$, while the evolving pairwise states predict both $v_A$ and $v_E$. Consequently, changes in atom representations, bond attributes, and connectivity are inferred from a shared evolving representation rather than from unrelated classification heads. The pairwise outputs are symmetrised for undirected graphs, and the complete vector field is permutation equivariant: $v_A(PAP^T, PX,PEP^T,t)=P\,v_A(A,X,E,t)\,P^T,$ with the corresponding transformations for $v_X$ and $v_E$. Therefore, node-relabelling consistency is respected at every infinitesimal ODE update, rather than being imposed only during final graph decoding.

The distinction from DiGress, DeFoG, and VFM is therefore both architectural and semantic. DiGress operates on discrete noisy graphs and predicts categorical denoising distributions over node and edge states. DeFoG similarly remains in a discrete graph state space and parameterises CTMC-based transition dynamics through discrete flow matching. VFM/CatFlow uses relaxed categorical states but predicts a categorical endpoint distribution from which its vector field is induced. Flowette instead introduces an edge-aware topology-conditioned transformer that directly predicts and integrates the coupled continuous velocities $(v_A,v_X,v_E)$. In particular, the simultaneous use of evolving soft adjacency as an attention bias, persistent dense pairwise states, separate adjacency and edge-attribute dynamics, and graph-consistent velocity outputs constitutes the novel architectural design.

We will revise the manuscript to state this claim more precisely.



Reviewer2 (nDMZ)
----
We sincerely thank for your valuable comments helping improve our work.

***Q1. Sensitivity to hand-designed graph priors.***

The graphette is intended as a structured source distribution, not as a substitute for the learned flow: it provides only coarse topology, such as rings, hubs, or acyclicity, while the velocity field learns the remaining target-specific structure. The performance drop under prior replacement therefore shows that a structurally compatible source reduces transport difficulty, rather than that the prior alone explains the final samples. 

Our controlled ablation in Appendix J.8.3 directly quantifies this sensitivity while keeping all other components fixed. Replacing the graphette with a motif-unaware standard graphon reduces QM9 validity from 99.81\% to 75.50\%, uniqueness from 99.30\% to 68.90\%, and increases NSPDK from 0.0003 to 0.0760. On ZINC250K, validity decreases from 99.90\% to 80.00\%, uniqueness from 100.00\% to 85.00\%, and NSPDK increases from 0.0006 to 0.0560. This experiment represents a stronger mismatch than merely disabling ring addition: it replaces the complete motif-aware molecular prior with a standard graphon. The result confirms that a structurally compatible source distribution substantially reduces the difficulty of the transport problem. We further quantify the **sensitivity of Flowette to graphette priors**; see our response to **Reviewer 8BQw, Question Q4**, for details.

The prior also need not remain manually specified. The base graphon $W$ could be estimated from data using implicit graphon-learning methods such as Implicit Graphon Neural Representation[1] or Scalable Implicit Graphon Learning[2]; the sparsification sequence $\rho_n$ could be fitted to empirical edge-density scaling; and the edit function $f$ could be selected or learned from motif statistics or validation performance. We use simple, interpretable priors here to isolate the contribution of structural source bias without introducing a second learned generator, and will clarify that automatic estimation of $W, \rho_n$, and $f$ is a natural extension of Flowette.

References
---
[1]Xia, Xinyue, Gal Mishne, and Yusu Wang. Implicit Graphon Neural Representation. AISTATS 2023.

[2]Azizpour, Ali, Nicolas Zilberstein, and Santiago Segarra. Scalable Implicit Graphon Learning. AISTATS 2025.

***Q2. Contribution of terminal projection vs. learned dynamics.***

We agree that the effect of terminal projection should be separated from that of the learned dynamics. We evaluated the same generated trajectories before and after valence-aware terminal projection, thereby isolating the contribution of post-processing from that of the learned dynamics.

|Dataset|Model Variant|Valid|Unique|Novel|Scaff|
|-|-|-|-|-|-|
|QM9|Pre-projection|98.06 $\pm$ 0.06|98.28 $\pm$ 0.07|98.00 $\pm$ 0.04|11.30|
||Post-projection|**99.81 $\pm$ 0.09**|**99.30 $\pm$ 0.05**|**99.10$\pm$ 0.06**|**13.60**|
|ZINC250K|Pre-projection|98.25$\pm$ 0.02|98.35$\pm$ 0.04|98.56$\pm$ 0.05|14.10|
||Post-projection|**99.90 $\pm$ 0.10**|**100.00 $\pm$ 0.0**|**100.00 $\pm$ 0.0**|**15.45**|
|MOSES|Pre-projection|97.95 $\pm$ 0.05|98.00 $\pm$ 0.03|97.06 $\pm$ 0.05|14.45|
||Post-projection|**99.05 $\pm$ 0.0**|**99.90 $\pm$ 0.0**|**98.10 $\pm$ 0.0**|**15.30**|

The pre-projection outputs already achieve high validity 98.06\% on QM9, 98.25\% on ZINC250K, and 97.95\% on MOSES, showing that the flow itself learns predominantly chemically feasible molecular structures. Projection provides only a modest additional improvement of 1.75, 1.65, and 1.10 percentage points, respectively, rather than transforming largely invalid outputs into valid molecules. Uniqueness and novelty also change only moderately, while scaffold scores remain close, indicating that projection corrects residual local valence violations without substantially redefining molecular identity or global structure. This is consistent with Flowette's training objective: the differentiable valence regulariser already encourages feasible endpoints during learning, whereas terminal projection acts as a final safeguard for occasional discretisation or finite-step integration errors.

Post-generation validity correction is not unique to Flowette. MoFlow[1] uses post-hoc validity correction when assembling generated molecular graphs, GraphEBM[2] applies validity correction to generated node and adjacency tensors, and autoregressive methods such as GraphAF[3] enforce validity checks during generation. However, we agree that the use of similar mechanisms in prior work does not by itself resolve the fairness concern. We therefore report Flowette's pre-projection metrics as the direct model-only comparison and its post-projection metrics separately as the performance of the complete generation pipeline. Applying exactly the same projection to a baseline is meaningful only when that method provides comparable atom- and bond-level confidence scores; otherwise, confidence-based bond correction would require an arbitrary ranking of discrete outputs and would not constitute an equivalent procedure. For baselines that expose compatible logits or probabilities, the same projection can be applied and evaluated directly.

References
---
[1]Chengxi et al., MoFlow: An Invertible Flow Model for Generating Molecular Graphs, KDD 2020

[2]Meng et al., GraphEBM: Molecular Graph Generation with Energy-Based Models, ICLR Workshop 2021

[3]Chence et al., GraphAF: a Flow-based Autoregressive Model for Molecular Graph Generation, ICLR 2020

***Q3. Continuous–discrete mismatch and test-time node sampling.***

Flowette does not assume that every intermediate continuous state corresponds to a chemically valid molecule or a literal sequence of graph edits; instead, the relaxed adjacency, atom-type, and bond-type tensors should be interpreted as soft confidence representations, analogous to class-probability vectors before categorical decoding. The relevant objective is therefore not to keep every intermediate point on the discrete graph space, but to learn a smooth transport whose endpoint lies close to a valid discrete graph. Flowette reduces this continuous–discrete gap through several complementary mechanisms: FGW coupling aligns source and target graphs according to both topology and node features, avoiding interpolation between arbitrarily mismatched structures; the molecular graphette prior already provides sparse, ring-enriched source graphs rather than unstructured noise; the GNN transformer evolves adjacency, atom types, and bond types jointly; and the endpoint-consistency, valence, and atom-marginal losses explicitly guide the terminal state toward a globally coherent and chemically feasible molecule. In particular, the endpoint loss directly supervises the graph predicted at $t=1$, while the theoretical analysis shows that accurate velocity and endpoint prediction yield exact endpoint recovery under the rectified-flow parameterisation, with finite-step errors controlled by velocity and integration errors. The ablations further support that validity is learned by the trajectory rather than produced only by post-processing, since removing endpoint or valence regularisation causes large validity drops despite using the same final projection. At inference, atom and bond features are decoded categorically and a lightweight valence-aware projection corrects only residual over-bonding. Node count is handled separately: Flowette learns a family of size-conditional transports $p_{\theta}(G|n)$ by matching source and target graphs with the same $n$; for unconditional generation, $n$ is first sampled from the empirical training node-count distribution, an $n$-node graphette is sampled, and the corresponding flow is integrated. Thus, training and generation are consistent.

***Q4. Scalability concerns. FGW coupling has nontrivial cost ($O(B^2 n^3)$).***

We add a controlled scaling study on Tree and SBM graphs with $n \in $ {$100,500,1000$}, using 2000 training-, 500 validation-, and 500 testing- graphs per setting. Trees are sampled from random Prufer sequences, while four-community SBMs use $p_{\mathrm{in}}=30/n$ and $p_{\mathrm{out}}=4/n$ to maintain approximately constant expected degree. Flowette supports the default online coupling protocol and two amortised variants (see our response to **Reviewer 8BQw, Question Q3**), fixed-pool and periodic coupling. We compare all three protocols under same hardware, model settings, and a 1000-epoch budget.

| Dataset | n | Online total (h) | Fixed-pool total (h) | Periodic total, K=10 (h)| 
|---|---:|---:|---:|---:|
|Tree|100|8.90|3.50|5.15|
||500|16.25|5.86|9.45|
||1000|26.30|8.67|12.36|
|SBM|100|12.25|5.65|7.91|
||500|22.05|8.82|12.75|
||1000|34.56|11.58|14.95|

We report the total end-to-end training time (i.e., FGW + Hungarian + model training). The scaling results show that repeatedly recomputing FGW introduces substantial training overhead, whereas amortising the coupling considerably improves practical scalability. Across Tree and SBM graphs, fixed-pool coupling reduces end-to-end training time by a large margin relative to online coupling, while periodic coupling with $K=10$ offers a smaller but still meaningful reduction, consistent with its role as an intermediate trade-off between full re-coupling and static correspondences. This consistent trend across both sparse, acyclic Trees and community-structured SBMs indicates that the benefit is not specific to a particular graph family. Fixed-pool coupling provides the lowest runtime, whereas periodic coupling offers an intermediate trade-off by refreshing the alignment during training. Importantly, neither FGW nor Hungarian matching is required at inference, so the associated computational overhead is confined to training.

***Q5. Role of the pretrained GIN encoder.***

We agree that the encoder's role should be highlighted more clearly; however, the requested sensitivity analysis is already provided in Appendix J.8.2 and Table 9.

% The encoder is a lightweight, self-supervised GIN graph autoencoder trained only on the training split and then frozen; it is used solely to define the intra-graph structural cost for FGW and does not participate in velocity-field learning, ODE integration, or inference. We compare four encoder conditions: the fully pretrained GIN, parameter-free three-iteration 1-WL structural features, an early-stopped GIN trained for only five epochs, and a randomly initialised frozen encoder. The training-free 1-WL alternative performs close to the pretrained GIN, for example, validity is 98.30\% versus 99.81\% on QM9 and 98.70\% versus 99.90\% on ZINC250K, whereas performance degrades progressively with the early-stopped and random encoders. This provides an important distinction: informative structural representations are indeed necessary for obtaining good FGW pairings, but Flowette's performance is not critically dependent on a highly optimised learned encoder, since a simple parameter-free structural descriptor remains competitive. Conversely, the degradation under weak or random encoders confirms the intended mechanism: when the structural cost becomes less meaningful, coupling quality and therefore velocity supervision deteriorate. We will make this existing ablation and the restricted role of the encoder more prominent in the main text.

% Reviewer 1: Q1
% We will revise Sec. 5.2 and the ablation discussion to state this explicitly: the fully-ablated variant is included as a domain-agnostic continuous-flow baseline, precisely to demonstrate that chemical feasibility does not emerge for free from architectural capacity or generic flow-matching supervision alone. Its degradation is evidence that our two chemistry-aware terms are targeted, low-overhead corrections for a specific and identifiable failure mode, not evidence that the underlying framework is bespoke to molecular data.

% The ablation in Table 8 is intentionally designed to demonstrate that these components address different failure modes rather than providing redundant improvements. The poor ablated performance does not indicate insufficient backbone capacity; it reflects a mismatch between coordinate-wise continuous velocity regression and the highly constrained, discrete nature of molecular graphs. Without $L_{end}$ and the chemistry-aware terms, the model is trained only to minimise average errors in relaxed adjacency, atom-type, and bond-type tensors. Such errors may be numerically small but chemically severe: changing one bond category or slightly overestimating one edge can violate valence and invalidate the entire molecule. A more expressive GNN can represent the desired velocity field, but architecture alone does not tell the model which continuous errors are chemically catastrophic. This contrasts with methods whose objectives are intrinsically aligned with categorical molecular variables: DiGress evolves discrete node and edge states and predicts categorical clean-graph distributions; DeFoG uses discrete flow matching with CTMC-based sampling; and VFM/CatFlow predicts a categorical endpoint distribution from which its vector field is induced. Their state spaces therefore provide stronger discrete inductive bias than plain continuous velocity regression. In Flowette, $L_{end}$ provides endpoint-aware temporal reweighting, while $L_{val}$ and $L_{atom}$ explicitly shape the endpoint toward feasible valence and atom composition. The ablated variant is therefore an intentionally unconstrained continuous-flow baseline, not the complete proposed method; its degradation demonstrates that sophisticated dynamics and chemistry-aware supervision are complementary rather than interchangeable.

% Reviewer 1: Q2

% We would revise the title and introduction to emphasise three complementary components: (i) graphettes as interpretable structural source priors requiring only coarse domain knowledge, (ii) FGW-based graph and node alignment for lower-variance supervision, and (iii) endpoint-aware and optional domain-specific regularisation for reliable discrete generation. We would also explicitly state that the chemistry losses are task-specific extensions rather than domain-agnostic contributions. The domain-agnostic claim would therefore be narrowed to the core framework, structured priors, coupling, and continuous transport, while acknowledging that the prior edit function and feasibility terms may use coarse domain knowledge and, for molecular data, task-specific losses. Structurally, we would introduce graphettes first, then FGW coupling, and finally the flow objective and regularisers, so the paper follows the actual generative pipeline, and so that what is fixed versus what is adapted per domain is visible from the outset rather than only reconstructable from the ablations and conclusion.

% We thank the reviewer for this constructive suggestion and agree that the paper should be framed more clearly around its integrated contribution to structurally reliable continuous graph flow matching, rather than presenting graphettes or the backbone as if they alone explain the full performance. We would state explicitly that Flowette is more domain-agnostic than many baselines, in particular, methods that build motif-specific structure directly into their architecture or state space, while relaxing our current bold claims to acknowledge that applying Flowette to a new domain still requires a coarse structural prior (the graphette edit function) and, for domains with hard combinatorial feasibility constraints, task-specific endpoint regularisers. 
% We will revise the title, abstract, introduction, and contribution summary to present Flowette as a domain-general generative core with lightweight domain-adaptive priors and constraints.

% We thank the reviewer for this constructive suggestion and agree that the paper should be framed around its integrated contribution to structurally reliable continuous flow matching for graphs. Importantly, Flowette's core components such as FGW-based coupling, the permutation-equivariant GNN transformer, and the core flow-matching objective ($L_{vel}$, $L_{end}$) remain entirely untouched across every experiment in the paper, synthetic and molecular alike; only the edit function, and for molecular data the chemistry-aware terms $L_{val}$ and $L_{atom}$, vary by domain.

% We thank the reviewer for this constructive suggestion and agree that the paper should be framed more clearly around its integrated contribution to structurally reliable continuous graph flow matching, rather than presenting graphettes or the backbone as if they alone explain the full performance. We would revise the title and introduction to emphasise three complementary components: (i) graphettes as interpretable structural source priors, (ii) FGW-based graph and node alignment for lower-variance supervision, and (iii) endpoint-aware and optional domain-specific regularisation for reliable discrete generation. We would also explicitly state that the chemistry losses are task-specific extensions rather than domain-agnostic contributions. The domain-agnostic claim would therefore be narrowed to the core framework, structured priors, coupling, and continuous transport, while acknowledging that the prior edit function and feasibility terms may use coarse domain knowledge. Structurally, we would introduce graphettes first, then FGW coupling, and finally the flow objective and regularisers, so the paper follows the actual generative pipeline.


% Reviewr 1 -> Q1

% A more expressive GNN may be capable of representing the correct velocity field, but capacity is not the central issue: a regression objective penalises residuals according to their numerical magnitude, even though their chemical consequences can differ substantially.

% The poor performance of the ablated variant does not reflect insufficient backbone capacity, it isolates a specific and well-understood mismatch between continuous velocity regression and the discrete, highly constrained nature of molecular graphs. Concretely, a numerically small error in a single bond-type logit can flip a single bond to a double bond, which is enough to violate valence and invalidate an entire molecule, while an error of similar magnitude elsewhere in the same graph is chemically inconsequential. A more expressive GNN can certainly represent the correct velocity field, the issue is not what the model can express, but that plain regression treats all residuals as equally costly, when chemically they are not.

==> appeal.tex <==
Reference 1
-----
Reference number or identifier in your paper: 57

Exact citation as it appears in the outcome of the citation checker:
H. Shirzad, H. Hajimirsadeghi, A. H. Abdi, and G. Mori. Td-gen: Graph generation with tree decomposition. Proceedings of the 25th International Conference on Artificial Intelligence and Statistics (AISTATS 2022).

Link to a public authoritative source for the citation format you used. Examples may include the publisher's website, official conference proceedings, journal page, arXiv, google scholars:
https://proceedings.mlr.press/v151/shirzad22a/shirzad22a.pdf

Basis for your appeal:
We acknowledge that the publication venue in this citation is incorrect. However, the referenced work itself is genuine: the title, authors, and year identify the existing TD-GEN paper. The authoritative PMLR record confirms that Hamed Shirzad, Hossein Hajimirsadeghi, Amir H. Abdi, and Greg Mori published TD-GEN: Graph Generation Using Tree Decomposition at AISTATS 2022. Therefore, the error concerns the publication venue rather than the existence or authorship of the cited work. Under the provided criteria, an incorrect venue that nevertheless exists is a minor bibliographic error and should not cause the reference to be classified as hallucinated.

Reference 2
-----
Reference number or identifier in your paper: 56

Exact citation as it appears in the outcome of the citation checker:
Omar Mahmood, Elman Mansimov, Richard Bonneau, and Kyunghyun Cho. Masked graph modeling for molecule generation. Nature communications, 2021.

Link to a public authoritative source for the citation format you used. Examples may include the publisher's website, official conference proceedings, journal page, arXiv, google scholars:
https://www.nature.com/articles/s41467-021-23415-2

Basis for your appeal:
We acknowledge that this reference contains incorrect bibliographic metadata. However, we respectfully request reconsideration of its classification as a hallucinated reference. The cited title, "Masked Graph Modeling for Molecule Generation", corresponds to a genuine and publicly verifiable publication. This reference was added at a late stage of manuscript preparation to strengthen the introduction and related work. Unfortunately, during this process, its bibliographic information was inadvertently cross-assigned with that of another genuine work in the same molecular graph generation literature, and we did not identify this error during our final reference checks. We fully acknowledge that this was an honest mistake on our part and that the reference should have been checked more carefully before submission. Importantly, however, the cited publication itself is genuine, identifiable from its title, and directly relevant to the discussion for which it was cited. The error therefore arose from an inadvertent association of metadata between existing publications rather than the fabrication of a nonexistent publication or scientific evidence. We respectfully ask that the nature and circumstances of this error be considered when determining whether this reference should be classified as hallucinated.

==> rebuttal_neurips.tex <==
Reviewer3 (8BQw)
----
We sincerely thank for your valuable comments helping improve our work.

***Q1. Node-level alignment induced by FGW is under-specified.***

In Flowette, FGW is used at two distinct levels: the scalar FGW distance $D_{ij}$ is used by the Hungarian algorithm to select graph-level source–target pairs, while the corresponding optimal transport plan $T_{ij}^{*}$ is subsequently used as a soft node-level alignment; it is neither discarded nor converted into a hard permutation. For a selected pair, we row-normalise the coupling to obtain $R_{ab}=\frac{T_{ab}^{\*}}{\sum_{b'}T_{ab'}^{\*}},$ where $R_{ab}$ represents the correspondence between source node $a$ and target node $b$. We row-normalise $T^{\*}$ because it represents joint transport mass; normalisation converts each row into a probability distribution over target nodes, preserving feature scale and recovering the exact permutation when the coupling is hard. Before forming any interpolants or velocity targets, the target graph is transported into the source-node coordinate system as, 

$\widetilde{X}_1 = R X_1$, 

$\widetilde{A}_1 = R A_1 R^{T}$, 

$\widetilde{E}_{1,ab:} = \sum\_{ab} R\_{aj} E\_{1,jk:} R\_{bk}$.

The flow is therefore constructed as $G_t=(1-t)G_0+t\widetilde{G}_1$, and the supervised velocities are $\widetilde{A}_1-A_0$, $\widetilde{X}_1-X_0$, and $\widetilde{E}_1-E_0;$ raw target ordering is never directly subtracted from the source ordering. We will revise the Algorithm 6 to explicitly insert this step between tensor construction and interpolation.

***Q2. Endpoint consistency loss may be less independent than claimed.***

We thank the reviewer for this precise observation and agree that our description of $L\_{end}$ as an independent global-consistency signal overstated its independence. Indeed, since $A_t = (1-t) A_0 + t A_1$, $\Delta A = A_1 - A_0$, and $\hat{A}_1 = A_t + (1-t)v_A$, we have $\hat{A}_1-A_1 = (1-t)(v_A-\Delta A)$ with identical relations for node and edge features. Thus, the endpoint term should be interpreted more precisely as an endpoint-aware temporal reweighting of velocity supervision, rather than as an independent source of global information. We will revise Sec. 3.3 to remove the "global transport consistency" framing and instead describe $L\_{end}$ as an algebraically induced, non-uniform temporal reweighting of the same velocity residual.

This reweighting is not arbitrary: the factor $(1−t)^2$ follows directly from the remaining extrapolation horizon in the one-step endpoint estimate, since the same velocity residual induces a larger predicted endpoint error when evaluated earlier in the trajectory. Theorem E.5 separately establishes that endpoint error under $K$-step Euler integration is controlled by velocity approximation error and numerical step size; it does not establish the independence of $L\_{end}$. Therefore, although $L\_{end}$ does not introduce a new supervision target, combining it with $\beta_\{end}$ provides an endpoint-aware temporal reweighting that places greater emphasis on velocity residuals having a larger immediate effect on the predicted terminal state.

***Q3. Runtime and precomputation claims need clarification.***

We support three explicit coupling protocols, and the default protocol Algorithm 1 is online coupling. Thus, the default method does not assume a fixed precomputed source pool. We additionally use two optional amortised variants: fixed-pool, which makes one blockwise pass over the training set before the first epoch, samples one source graph per target, stores the corresponding source graph and FGW transport plan keyed by the target index, and reuses them across all epochs; and periodic, which refreshes this cache every $K$ epochs. Importantly, pre-computation is performed in minibatch-sized $B \times B$ blocks rather than as a single dataset-wide matching problem, and the cached correspondence remains valid under shuffled training because it is indexed by the target graph's dataset index. We will therefore revise the paper to state explicitly those protocols and avoid conflating the default online procedure with the optional amortised version: under online coupling, FGW cost is paid every minibatch and epoch, whereas under fixed-pool coupling it is a one-time preprocessing cost that is reused throughout training.

***Q4. Manual graphette specification and finite-graph approximation.***

The graphette prior could be made more data-driven: the base graphon $W$ could be estimated using graphon learning or implicit neural representation methods, $\rho_n$ could be fitted to match the empirical edge-density scaling conditional on $n$, and the edit distribution $f$ could be learned from motif statistics rather than selected manually. We deliberately use simple, interpretable priors in the present work because the graphette is only the source distribution of the flow, not the final generative model; it is intended to provide a coarse structural bias, such as rings, hubs, or acyclicity, while the velocity field learns the remaining target-specific structure. This also lets us isolate the benefit of structural source bias without introducing a second learned generator.

Sensitivity is partly quantified by our controlled ablation in Appendix J.8.3, where the graphette is replaced by a standard graphon. On QM9, validity and uniqueness decrease from 99.81\% and 99.30\% to 75.50\% and 68.90\%, respectively, while NSPDK increases from 0.0003 to 0.0760; analogous degradation occurs on ZINC250K. This confirms that a structurally compatible prior is important, but we agree that this is an extreme removal ablation rather than a complete misspecification study. 

To further quantify **sensitivity to graphette misspecification**, we performed a controlled experiment as in the following table which all components of Flowette were kept fixed, while only the edit function $f$ was changed. For molecular datasets, the original Flowette prior uses ring addition $R$, reflecting the prevalence of cyclic structures in molecules; we compare it against the structurally incompatible star-addition edit $S$ and the contradictory cycle-deletion edit $h$. The results show a clear and consistent degradation as the prior becomes less compatible with the target domain: on QM9, replacing $R$ with $S$ reduces validity from 99.81\% to 70.50\%, while cycle deletion further reduces it to 53.70\%; analogous trends are observed on ZINC250K, together with substantial increases in NSPDK. This demonstrates that Flowette benefits from a coarse but structurally appropriate source prior and is sensitive to motif misspecification, rather than being invariant to the choice of graphette edit. 
|Dataset|Edit function|Prior variant|Valid|Unique|NSPDK|
|-|-|-|-|-|-|
|QM9|R (Ring addition)|Intended prior|**99.81 $\pm$ 0.09**|**99.30 $\pm$ 0.05**|**0.0003 $\pm$ 0.002**|
||S (Star addition)|Incorrect motif|70.50 $\pm$ 0.06|69.30 $\pm$ 0.06|0.0160 $\pm$ 0.008|
||h (Cycle deletion)|Contradictory motif|53.70 $\pm$ 0.04|54.45 $\pm$ 0.06|0.0540 $\pm$ 0.004|
|ZINC250K|R (Ring addition)|Intended prior|**99.90 $\pm$ 0.10**|**100.00 $\pm$ 0.0**|**0.0006 $\pm$ 0.004**|
||S (Star addition)|Incorrect motif|73.40 $\pm$ 0.06|75.30 $\pm$ 0.06|0.1105 $\pm$ 0.006|
||h (Cycle deletion)|Contradictory motif|51.58 $\pm$ 0.04|50.65 $\pm$ 0.05|0.2050 $\pm$ 0.007|

***Q5. Minor: FGW vs GW.***

We agree that standard GW is sufficient for genuinely non-attributed graphs, and FGW naturally recovers this setting: in Eq. (4), $\alpha=1$ gives GW exactly, while absent or constant node features make the feature term non-discriminative. Our motivation for FGW is therefore not to outperform GW on purely structural datasets, but to provide a unified coupling that also handles attributed graphs. This becomes important for molecules, where topology alone may align structurally similar but chemically incompatible atoms, leading to noisy feature interpolation and velocity targets; FGW resolves this ambiguity by jointly matching topology and atom identity.

To isolate the feature contribution, we compared FGW ($\alpha=0.5$) with GW ($\alpha=1.0$) while keeping all other components fixed. As expected, their performance is essentially identical on the non-attributed Tree and SBM benchmarks: both achieve 100\% validity, uniqueness, novelty, and V.U.N, with only negligible differences in structural MMD metrics. These results confirm that FGW behaves like GW when attributes are uninformative, while retaining the flexibility needed for attributed molecular graphs.

|Dataset|Model Variant|Deg|Clus.|Orbit|Valid|Unique|Novel|V.U.N|
|-|-|-|-|-|-|-|-|-|
|Tree|Flowette (FGW)|0.00005$\pm$ 0.002|0.0000$\pm$ 0.0|0.0000$\pm$ 0.0|100.0$\pm$ 0.0|100.0$\pm$ 0.0|100.0$\pm$ 0.0|100.0$\pm$ 0.0|
||Flowette (GW)|0.00010$\pm$ 0.003|0.0000$\pm$ 0.0|0.0000$\pm$ 0.0|100.0$\pm$ 0.0|100.0$\pm$ 0.0|100.0$\pm$ 0.0|100.0$\pm$ 0.0|
|SBM|Flowette (FGW)|0.0076$\pm$ 0.003|0.0508$\pm$ 0.01|0.0000$\pm$ 0.0|100.0$\pm$ 0.0|100.0$\pm$ 0.0|100.0$\pm$ 0.0|100.0$\pm$ 0.0|
||Flowette (GW)|0.0080$\pm$ 0.005|0.0595$\pm$ 0.03|0.0000$\pm$ 0.0|100.0$\pm$ 0.0|100.0 $\pm$ 0.0|100.0$\pm$ 0.0|100.0$\pm$ 0.0|




Reviewer1 (9NKx)
----
We sincerely thank the reviewer for valuable comments.

***Q1. Why does the velocity-only model perform poorly on molecules?***

Let us clarify an important distinction that Table 8 alone does not fully convey. The poor performance of the ablated variant does not reflect insufficient backbone capacity, it isolates a specific and well-understood mismatch between continuous velocity regression and the discrete, highly constrained nature of molecular graphs. Concretely, a numerically small error in a single bond-type logit can flip a single bond to a double bond, which is enough to violate valence and invalidate an entire molecule, while an error of similar magnitude elsewhere in the same graph is chemically inconsequential. A more expressive GNN can certainly represent the correct velocity field, the issue is not what the model can express, but the regression treats all residuals as equally costly, when chemically they are not.

Crucially, this mismatch is specific to the molecular setting, not a general weakness of our framework. The same backbone - FGW-coupled supervision, the permutation-equivariant GNN transformer, and the rectified flow-matching objective, achieves SOTA results on our synthetic benchmarks (Tree, SBM, Ego-small) with $\beta_{val}=\beta_{atom}=0$ and no chemistry terms whatsoever. The backbone is therefore already domain-general and demonstrably strong on its own; it is only when the target domain has hard combinatorial constraints, like valence, that additional supervision is needed to align the training signal with what correct means in that domain.

Methods like DiGress, DeFoG, and VFM/CatFlow address this problem by building their entire generative process around categorical/discrete state spaces from the ground up. We instead retain the general continuous-flow backbone and attach two lightweight, differentiable regularizers at the predicted endpoint, $L_{val}$ and $L_{atom}$, that penalize exactly the failure mode described above. These require only coarse, easily specified domain knowledge, valence limits and target atom-type marginals, and negligible architectural or computational overhead (Appendix D, F). This is an addition to a general model, not a redesign of it: the coupling mechanism, network architecture, and core flow-matching objective are shared unchanged between our synthetic and molecular experiments, and the domain-specific surface area is confined to these two interpretable terms.

We will revise Sec. 5.2 to state this explicitly: the ablated variant shows that chemical feasibility does not emerge for free from architecture or generic flow-matching supervision alone, evidence that our two chemistry-aware terms are targeted, low-overhead corrections for a specific failure mode, not that the framework is bespoke to molecular data.

***Q2. Misalignment between framing and actual contributions.***

We thank the reviewer for this constructive suggestion and agree that the paper should be framed around its integrated contribution to structurally reliable continuous flow matching for graphs, rather than implying that either graphettes or the backbone alone explains the final performance. Importantly, Flowette retains the same core formulation across synthetic and molecular experiments: FGW-based graph- and node-level coupling, the permutation-equivariant continuous velocity-field GNN, and the flow-matching objectives $L_{vel}$ and $L_{end}$. Domain adaptation occurs only through the coarse graphette edit function and, for molecular datasets, the chemistry-aware regularisers $L_{val}$ and $L_{atom}$.

We will revise the title, introduction, and contribution summary to emphasise three complementary components: (i) graphettes as interpretable structural source priors requiring only coarse domain knowledge, (ii) FGW-based graph- and node-level alignment that provides topology-aware supervision, and (iii) endpoint-aware training with optional domain-specific feasibility regularisation for discrete graph generation. We will explicitly distinguish the reusable, domain-general core-coupling, continuous transport, and the velocity-field architecture from the domain-adaptive prior and chemistry-aware feasibility constraints.

We will also restructure the paper to follow the generative pipeline: graphette construction first, followed by FGW coupling, the continuous flow model, and finally the optional regularisers. This ordering will make clear from the outset which components are shared across domains and which are adapted to a particular task, rather than leaving this distinction to be inferred from the ablations and limitations.

***Q3. What distinguishes GNN backbone from existing graph transformer architectures.***

We thank the reviewer for requesting this clarification. We do claim that the GNN Transformer is a novel architecture. While existing graph transformers operate on fixed discrete states predicting node/edge categories, ours fundamentally differs in three ways: (1) it operates on continuous evolving triple-representations $(A_t, X_t, E_t)$ , predicting velocity fields $(v_A, v_X, v_E)$ rather than categorical outputs; (2) it maintains pairwise edge hidden states with soft adjacency $A_t$ injected as a structural bias in attention logits, absent in existing transformers; and (3) velocity outputs are explicitly symmetrised with time embedding jointly conditioning both node and edge dynamics, unique to continuous flow matching. Together, these make our architecture an original contribution tailored to continuous-time flow matching on attributed graphs.

**(1) Joint continuous graph state and direct velocity prediction.**  Flowette operates on the continuously relaxed graph state $G_t=(A_t,X_t,E_t)$ and directly predicts the coupled velocity field $v_\theta(G_t,t)=(v_A,v_X,v_E)$, where adjacency, node attributes, and edge attributes evolve simultaneously. These outputs are tangent directions that are repeatedly evaluated and integrated by the ODE solver, rather than categorical clean-state logits, endpoint probabilities, or discrete transition rates. The network must therefore remain meaningful throughout the continuum of fractional graph states encountered during generation, not only at discrete valid graphs.

**(2) Explicit separation of evolving topology and edge attributes.**  
Flowette treats soft connectivity $A_t(i,j)$ and edge attributes $E_t(i,j)$ as related but distinct evolving variables. The current soft adjacency is inserted directly into the attention logits, $S_{ij}^{(\ell)} = \frac{\langle Q_i^{(\ell)},K_j^{(\ell)}\rangle}{\sqrt{H}} + A_t(i,j)$, so the evolving topology continuously modulates information exchange. In parallel, a separate pairwise hidden state $b_{ij}^{(\ell)}$, initialised from $E_t$, participates in message construction and is updated at every layer. Thus, $A_t$ controls where and how strongly nodes communicate, while the pairwise state represents what edge-specific information is exchanged. This separation is particularly relevant for molecular graphs because bond existence and bond type are strongly related but are not identical variables.

**(3) Time conditions the complete topology–attribute dynamics.**  
The time embedding is injected into both node and pairwise representations, allowing the interaction between topology and attributes to change throughout transport. Near $t=0$, the field performs coarse transformations from a graphette-prior sample, whereas near $t=1$, it performs finer structural and attribute corrections. Time therefore does not merely serve as a denoising-step index; it conditions a single continuous vector field whose outputs define the right-hand side of the graph ODE.

**(4) Coupled and graph-consistent infinitesimal updates.**  
The final node states predict $v_X$, while the evolving pairwise states predict both $v_A$ and $v_E$. Consequently, changes in atom representations, bond attributes, and connectivity are inferred from a shared evolving representation rather than from unrelated classification heads. The pairwise outputs are symmetrised for undirected graphs, and the complete vector field is permutation equivariant: $v_A(PAP^T, PX,PEP^T,t)=P\,v_A(A,X,E,t)\,P^T,$ with the corresponding transformations for $v_X$ and $v_E$. Therefore, node-relabelling consistency is respected at every infinitesimal ODE update, rather than being imposed only during final graph decoding.

The distinction from DiGress, DeFoG, and VFM is therefore both architectural and semantic. DiGress operates on discrete noisy graphs and predicts categorical denoising distributions over node and edge states. DeFoG similarly remains in a discrete graph state space and parameterises CTMC-based transition dynamics through discrete flow matching. VFM/CatFlow uses relaxed categorical states but predicts a categorical endpoint distribution from which its vector field is induced. Flowette instead introduces an edge-aware topology-conditioned transformer that directly predicts and integrates the coupled continuous velocities $(v_A,v_X,v_E)$. In particular, the simultaneous use of evolving soft adjacency as an attention bias, persistent dense pairwise states, separate adjacency and edge-attribute dynamics, and graph-consistent velocity outputs constitutes the novel architectural design.

We will revise the manuscript to state this claim more precisely.



Reviewer2 (nDMZ)
----
We sincerely thank for your valuable comments helping improve our work.

***Q1. Sensitivity to hand-designed graph priors.***

The graphette is intended as a structured source distribution, not as a substitute for the learned flow: it provides only coarse topology, such as rings, hubs, or acyclicity, while the velocity field learns the remaining target-specific structure. The performance drop under prior replacement therefore shows that a structurally compatible source reduces transport difficulty, rather than that the prior alone explains the final samples. 

Our controlled ablation in Appendix J.8.3 directly quantifies this sensitivity while keeping all other components fixed. Replacing the graphette with a motif-unaware standard graphon reduces QM9 validity from 99.81\% to 75.50\%, uniqueness from 99.30\% to 68.90\%, and increases NSPDK from 0.0003 to 0.0760. On ZINC250K, validity decreases from 99.90\% to 80.00\%, uniqueness from 100.00\% to 85.00\%, and NSPDK increases from 0.0006 to 0.0560. This experiment represents a stronger mismatch than merely disabling ring addition: it replaces the complete motif-aware molecular prior with a standard graphon. The result confirms that a structurally compatible source distribution substantially reduces the difficulty of the transport problem. We further quantify the **sensitivity of Flowette to graphette priors**; see our response to **Reviewer 8BQw, Question Q4**, for details.

The prior also need not remain manually specified. The base graphon $W$ could be estimated from data using implicit graphon-learning methods such as Implicit Graphon Neural Representation[1] or Scalable Implicit Graphon Learning[2]; the sparsification sequence $\rho_n$ could be fitted to empirical edge-density scaling; and the edit function $f$ could be selected or learned from motif statistics or validation performance. We use simple, interpretable priors here to isolate the contribution of structural source bias without introducing a second learned generator, and will clarify that automatic estimation of $W, \rho_n$, and $f$ is a natural extension of Flowette.

References
---
[1]Xia, Xinyue, Gal Mishne, and Yusu Wang. Implicit Graphon Neural Representation. AISTATS 2023.

[2]Azizpour, Ali, Nicolas Zilberstein, and Santiago Segarra. Scalable Implicit Graphon Learning. AISTATS 2025.

***Q2. Contribution of terminal projection vs. learned dynamics.***

We agree that the effect of terminal projection should be separated from that of the learned dynamics. We evaluated the same generated trajectories before and after valence-aware terminal projection, thereby isolating the contribution of post-processing from that of the learned dynamics.

|Dataset|Model Variant|Valid|Unique|Novel|Scaff|
|-|-|-|-|-|-|
|QM9|Pre-projection|98.06 $\pm$ 0.06|98.28 $\pm$ 0.07|98.00 $\pm$ 0.04|11.30|
||Post-projection|**99.81 $\pm$ 0.09**|**99.30 $\pm$ 0.05**|**99.10$\pm$ 0.06**|**13.60**|
|ZINC250K|Pre-projection|98.25$\pm$ 0.02|98.35$\pm$ 0.04|98.56$\pm$ 0.05|14.10|
||Post-projection|**99.90 $\pm$ 0.10**|**100.00 $\pm$ 0.0**|**100.00 $\pm$ 0.0**|**15.45**|
|MOSES|Pre-projection|97.95 $\pm$ 0.05|98.00 $\pm$ 0.03|97.06 $\pm$ 0.05|14.45|
||Post-projection|**99.05 $\pm$ 0.0**|**99.90 $\pm$ 0.0**|**98.10 $\pm$ 0.0**|**15.30**|

The pre-projection outputs already achieve high validity 98.06\% on QM9, 98.25\% on ZINC250K, and 97.95\% on MOSES, showing that the flow itself learns predominantly chemically feasible molecular structures. Projection provides only a modest additional improvement of 1.75, 1.65, and 1.10 percentage points, respectively, rather than transforming largely invalid outputs into valid molecules. Uniqueness and novelty also change only moderately, while scaffold scores remain close, indicating that projection corrects residual local valence violations without substantially redefining molecular identity or global structure. This is consistent with Flowette's training objective: the differentiable valence regulariser already encourages feasible endpoints during learning, whereas terminal projection acts as a final safeguard for occasional discretisation or finite-step integration errors.

Post-generation validity correction is not unique to Flowette. MoFlow[1] uses post-hoc validity correction when assembling generated molecular graphs, GraphEBM[2] applies validity correction to generated node and adjacency tensors, and autoregressive methods such as GraphAF[3] enforce validity checks during generation. However, we agree that the use of similar mechanisms in prior work does not by itself resolve the fairness concern. We therefore report Flowette's pre-projection metrics as the direct model-only comparison and its post-projection metrics separately as the performance of the complete generation pipeline. Applying exactly the same projection to a baseline is meaningful only when that method provides comparable atom- and bond-level confidence scores; otherwise, confidence-based bond correction would require an arbitrary ranking of discrete outputs and would not constitute an equivalent procedure. For baselines that expose compatible logits or probabilities, the same projection can be applied and evaluated directly.

References
---
[1]Chengxi et al., MoFlow: An Invertible Flow Model for Generating Molecular Graphs, KDD 2020

[2]Meng et al., GraphEBM: Molecular Graph Generation with Energy-Based Models, ICLR Workshop 2021

[3]Chence et al., GraphAF: a Flow-based Autoregressive Model for Molecular Graph Generation, ICLR 2020

***Q3. Continuous–discrete mismatch and test-time node sampling.***

Flowette does not assume that every intermediate continuous state corresponds to a chemically valid molecule or a literal sequence of graph edits; instead, the relaxed adjacency, atom-type, and bond-type tensors should be interpreted as soft confidence representations, analogous to class-probability vectors before categorical decoding. The relevant objective is therefore not to keep every intermediate point on the discrete graph space, but to learn a smooth transport whose endpoint lies close to a valid discrete graph. Flowette reduces this continuous–discrete gap through several complementary mechanisms: FGW coupling aligns source and target graphs according to both topology and node features, avoiding interpolation between arbitrarily mismatched structures; the molecular graphette prior already provides sparse, ring-enriched source graphs rather than unstructured noise; the GNN transformer evolves adjacency, atom types, and bond types jointly; and the endpoint-consistency, valence, and atom-marginal losses explicitly guide the terminal state toward a globally coherent and chemically feasible molecule. In particular, the endpoint loss directly supervises the graph predicted at $t=1$, while the theoretical analysis shows that accurate velocity and endpoint prediction yield exact endpoint recovery under the rectified-flow parameterisation, with finite-step errors controlled by velocity and integration errors. The ablations further support that validity is learned by the trajectory rather than produced only by post-processing, since removing endpoint or valence regularisation causes large validity drops despite using the same final projection. At inference, atom and bond features are decoded categorically and a lightweight valence-aware projection corrects only residual over-bonding. Node count is handled separately: Flowette learns a family of size-conditional transports $p_{\theta}(G|n)$ by matching source and target graphs with the same $n$; for unconditional generation, $n$ is first sampled from the empirical training node-count distribution, an $n$-node graphette is sampled, and the corresponding flow is integrated. Thus, training and generation are consistent.

***Q4. Scalability concerns. FGW coupling has nontrivial cost ($O(B^2 n^3)$).***

We add a controlled scaling study on Tree and SBM graphs with $n \in $ {$100,500,1000$}, using 2000 training-, 500 validation-, and 500 testing- graphs per setting. Trees are sampled from random Prufer sequences, while four-community SBMs use $p_{\mathrm{in}}=30/n$ and $p_{\mathrm{out}}=4/n$ to maintain approximately constant expected degree. Flowette supports the default online coupling protocol and two amortised variants (see our response to **Reviewer 8BQw, Question Q3**), fixed-pool and periodic coupling. We compare all three protocols under same hardware, model settings, and a 1000-epoch budget.

| Dataset | n | Online total (h) | Fixed-pool total (h) | Periodic total, K=10 (h)| 
|---|---:|---:|---:|---:|
|Tree|100|8.90|3.50|5.15|
||500|16.25|5.86|9.45|
||1000|26.30|8.67|12.36|
|SBM|100|12.25|5.65|7.91|
||500|22.05|8.82|12.75|
||1000|34.56|11.58|14.95|

We report the total end-to-end training time (i.e., FGW + Hungarian + model training). The scaling results show that repeatedly recomputing FGW introduces substantial training overhead, whereas amortising the coupling considerably improves practical scalability. Across Tree and SBM graphs, fixed-pool coupling reduces end-to-end training time by a large margin relative to online coupling, while periodic coupling with $K=10$ offers a smaller but still meaningful reduction, consistent with its role as an intermediate trade-off between full re-coupling and static correspondences. This consistent trend across both sparse, acyclic Trees and community-structured SBMs indicates that the benefit is not specific to a particular graph family. Fixed-pool coupling provides the lowest runtime, whereas periodic coupling offers an intermediate trade-off by refreshing the alignment during training. Importantly, neither FGW nor Hungarian matching is required at inference, so the associated computational overhead is confined to training.

***Q5. Role of the pretrained GIN encoder.***

We agree that the encoder's role should be highlighted more clearly; however, the requested sensitivity analysis is already provided in Appendix J.8.2 and Table 9.

% The encoder is a lightweight, self-supervised GIN graph autoencoder trained only on the training split and then frozen; it is used solely to define the intra-graph structural cost for FGW and does not participate in velocity-field learning, ODE integration, or inference. We compare four encoder conditions: the fully pretrained GIN, parameter-free three-iteration 1-WL structural features, an early-stopped GIN trained for only five epochs, and a randomly initialised frozen encoder. The training-free 1-WL alternative performs close to the pretrained GIN, for example, validity is 98.30\% versus 99.81\% on QM9 and 98.70\% versus 99.90\% on ZINC250K, whereas performance degrades progressively with the early-stopped and random encoders. This provides an important distinction: informative structural representations are indeed necessary for obtaining good FGW pairings, but Flowette's performance is not critically dependent on a highly optimised learned encoder, since a simple parameter-free structural descriptor remains competitive. Conversely, the degradation under weak or random encoders confirms the intended mechanism: when the structural cost becomes less meaningful, coupling quality and therefore velocity supervision deteriorate. We will make this existing ablation and the restricted role of the encoder more prominent in the main text.

% Reviewer 1: Q1
% We will revise Sec. 5.2 and the ablation discussion to state this explicitly: the fully-ablated variant is included as a domain-agnostic continuous-flow baseline, precisely to demonstrate that chemical feasibility does not emerge for free from architectural capacity or generic flow-matching supervision alone. Its degradation is evidence that our two chemistry-aware terms are targeted, low-overhead corrections for a specific and identifiable failure mode, not evidence that the underlying framework is bespoke to molecular data.

% The ablation in Table 8 is intentionally designed to demonstrate that these components address different failure modes rather than providing redundant improvements. The poor ablated performance does not indicate insufficient backbone capacity; it reflects a mismatch between coordinate-wise continuous velocity regression and the highly constrained, discrete nature of molecular graphs. Without $L_{end}$ and the chemistry-aware terms, the model is trained only to minimise average errors in relaxed adjacency, atom-type, and bond-type tensors. Such errors may be numerically small but chemically severe: changing one bond category or slightly overestimating one edge can violate valence and invalidate the entire molecule. A more expressive GNN can represent the desired velocity field, but architecture alone does not tell the model which continuous errors are chemically catastrophic. This contrasts with methods whose objectives are intrinsically aligned with categorical molecular variables: DiGress evolves discrete node and edge states and predicts categorical clean-graph distributions; DeFoG uses discrete flow matching with CTMC-based sampling; and VFM/CatFlow predicts a categorical endpoint distribution from which its vector field is induced. Their state spaces therefore provide stronger discrete inductive bias than plain continuous velocity regression. In Flowette, $L_{end}$ provides endpoint-aware temporal reweighting, while $L_{val}$ and $L_{atom}$ explicitly shape the endpoint toward feasible valence and atom composition. The ablated variant is therefore an intentionally unconstrained continuous-flow baseline, not the complete proposed method; its degradation demonstrates that sophisticated dynamics and chemistry-aware supervision are complementary rather than interchangeable.

% Reviewer 1: Q2

% We would revise the title and introduction to emphasise three complementary components: (i) graphettes as interpretable structural source priors requiring only coarse domain knowledge, (ii) FGW-based graph and node alignment for lower-variance supervision, and (iii) endpoint-aware and optional domain-specific regularisation for reliable discrete generation. We would also explicitly state that the chemistry losses are task-specific extensions rather than domain-agnostic contributions. The domain-agnostic claim would therefore be narrowed to the core framework, structured priors, coupling, and continuous transport, while acknowledging that the prior edit function and feasibility terms may use coarse domain knowledge and, for molecular data, task-specific losses. Structurally, we would introduce graphettes first, then FGW coupling, and finally the flow objective and regularisers, so the paper follows the actual generative pipeline, and so that what is fixed versus what is adapted per domain is visible from the outset rather than only reconstructable from the ablations and conclusion.

% We thank the reviewer for this constructive suggestion and agree that the paper should be framed more clearly around its integrated contribution to structurally reliable continuous graph flow matching, rather than presenting graphettes or the backbone as if they alone explain the full performance. We would state explicitly that Flowette is more domain-agnostic than many baselines, in particular, methods that build motif-specific structure directly into their architecture or state space, while relaxing our current bold claims to acknowledge that applying Flowette to a new domain still requires a coarse structural prior (the graphette edit function) and, for domains with hard combinatorial feasibility constraints, task-specific endpoint regularisers. 
% We will revise the title, abstract, introduction, and contribution summary to present Flowette as a domain-general generative core with lightweight domain-adaptive priors and constraints.

% We thank the reviewer for this constructive suggestion and agree that the paper should be framed around its integrated contribution to structurally reliable continuous flow matching for graphs. Importantly, Flowette's core components such as FGW-based coupling, the permutation-equivariant GNN transformer, and the core flow-matching objective ($L_{vel}$, $L_{end}$) remain entirely untouched across every experiment in the paper, synthetic and molecular alike; only the edit function, and for molecular data the chemistry-aware terms $L_{val}$ and $L_{atom}$, vary by domain.

% We thank the reviewer for this constructive suggestion and agree that the paper should be framed more clearly around its integrated contribution to structurally reliable continuous graph flow matching, rather than presenting graphettes or the backbone as if they alone explain the full performance. We would revise the title and introduction to emphasise three complementary components: (i) graphettes as interpretable structural source priors, (ii) FGW-based graph and node alignment for lower-variance supervision, and (iii) endpoint-aware and optional domain-specific regularisation for reliable discrete generation. We would also explicitly state that the chemistry losses are task-specific extensions rather than domain-agnostic contributions. The domain-agnostic claim would therefore be narrowed to the core framework, structured priors, coupling, and continuous transport, while acknowledging that the prior edit function and feasibility terms may use coarse domain knowledge. Structurally, we would introduce graphettes first, then FGW coupling, and finally the flow objective and regularisers, so the paper follows the actual generative pipeline.


% Reviewr 1 -> Q1

% A more expressive GNN may be capable of representing the correct velocity field, but capacity is not the central issue: a regression objective penalises residuals according to their numerical magnitude, even though their chemical consequences can differ substantially.

% The poor performance of the ablated variant does not reflect insufficient backbone capacity, it isolates a specific and well-understood mismatch between continuous velocity regression and the discrete, highly constrained nature of molecular graphs. Concretely, a numerically small error in a single bond-type logit can flip a single bond to a double bond, which is enough to violate valence and invalidate an entire molecule, while an error of similar magnitude elsewhere in the same graph is chemically inconsequential. A more expressive GNN can certainly represent the correct velocity field, the issue is not what the model can express, but that plain regression treats all residuals as equally costly, when chemically they are not.
